Causal Effect Regularization: Automated Detection and Removal of Spurious Attributes

In many classification datasets, the task labels are spuriously correlated with some input attributes. Classifiers trained on such datasets often rely on these attributes for prediction, especially when the spurious correlation is high, and thus fail to generalize whenever there is a shift in the attributes' correlation at deployment. If we assume that the spurious attributes are known a priori, several methods have been proposed to learn a classifier that is invariant to the specified attributes. However, in real-world data, information about spurious attributes is typically unavailable. Therefore, we propose a method to automatically identify spurious attributes by estimating their causal effect on the label and then use a regularization objective to mitigate the classifier's reliance on them. Compared to a recent method for identifying spurious attributes, we find that our method is more accurate in removing the attribute from the learned model, especially when spurious correlation is high. Specifically, across synthetic, semi-synthetic, and real-world datasets, our method shows significant improvement in a metric used to quantify the dependence of a classifier on spurious attributes ($\Delta$Prob), while obtaining better or similar accuracy. In addition, our method mitigates the reliance on spurious attributes even under noisy estimation of causal effects. To explain the empirical robustness of our method, we create a simple linear classification task with two sets of attributes: causal and spurious. We prove that our method only requires that the ranking of estimated causal effects is correct across attributes to select the correct classifier.

==> sections/outline.tex <==
\section{Outline: Temporary}
\paragraph{Motivation and Problem}
\begin{enumerate}
    \item Problem: Generalization wrt the change in the distribution of spuriously correlated attributes. 
    \begin{enumerate}
        \item 
    \end{enumerate}
    \item Most of the existing methods that aim to remove the reliance of the model on spurious correlations assume the knowledge of spuriously correlated attributes.

    \item Our Problem: Given a task and a set of high-level concepts/attributes which are correlated with the task labels:
    \begin{enumerate}
        \item How can we automatically discover the spuriously correlated attributes?
        
        \item How can we regularize the model to remove the reliance on spuriously correlated attributes even with a noisy estimate of spurious attributes?\amits{need to prime the reader first why noise is an issue. we should say that due to identification issues, spurious features may not be fully identified. so some noise/error is expected. so any method  should be robust to that}
    \end{enumerate}

\end{enumerate}
\amits{The above description is good. You may also want to say that this problem is called by different names, e,g.,  transformation from Mouli et al and ``intervention'' by other work, and say that all of this mean the same thing and we are solving all these problems.}
\paragraph{Comparison and How we are situated wrt to previous work}
\begin{enumerate}
    \item Current State: Most of the current methods: 
    \begin{enumerate}
        \item directly assumes knowledge of spuriously correlated labels or uses human annotation: \cite{kaushik2021learningthediff,victorStressTest,GroupDRO}.

        \item indirectly in the form of multiple environments \cite{IRM:2020}.

        \item assumes invariance with respect to certain transformations \cite{AutoAugment_2019_CVPR}. \abhinav{cite Andrew's work on automatically discovering symmetry}

        \item Automatically finding invariances \cite{mouli2022asymmetry,mouli2021neural} but under certain assumptions and generalize to limited settings or kinds of distribution shifts. \amits{what are these limited settings? let's create a good argument against mouli}
    \end{enumerate}

    \item How we are different:
    \begin{enumerate}
        \item Identifying causal vs spurious attributes (Stage 1):
        \begin{enumerate}
            \item Uses off-the-shelf causal effect estimators. Zero causal effect $\implies$ the attribute is spurious. The identifiability assumptions are the same as the chosen estimator. \amits{need to say more. Since we assume access to CF example, does it help with identifiability? Is no unobserved confounding likely to hold? good to provide an identification result as a proposition and list assumptions needed.}
            \begin{enumerate}
                \item We make an additional assumption that we have access to the counterfactual example i.e. give (X(T=t), Y) we have access to X(T=t') where the topic value is changed from t to t'. 
            \end{enumerate}
            \amits{do we also need to argue that not all features may be spurious and our method helps to avoid hardcoding/setting the effect to zero?}
        \end{enumerate}
    
    
        \item Regularizing the models (Stage 2):
        \begin{enumerate}
            \item New regularization objective to train a robust model using the estimated treatment effect.\amits{what is the novelty in regularization objective? The hard constraint seems like a fairly obvious regularizer once we know the causal effect.}

            \item Analysis (theory + empirical) on the robustness of the proposed method with noise in the estimated treatment effect. 
        \end{enumerate}
    
    
        \item Limitations:
        \begin{enumerate}
            \item Will not work in an anti-causal task setting. 
            \item 
        \end{enumerate}
    \end{enumerate}

\end{enumerate}


\paragraph{Main Claims to prove our point}
\amits{Story: I see a recurring message that can be the main message we highlight: Our method is perfect under no-confounding, but even with confounding,  our method is reasonably robust.}
\begin{enumerate}
    \item Datasets:
    \begin{enumerate}
        \item SyntheticText: (NLP dataset)
        \begin{enumerate}
            \item  has 3 topics (causal, spurious, and confound) where we can artificially vary the correlation of spurious features with the main task label.

            \item For every topic, we have a set of words that are then concatenated to create the example sentence.  The counterfactuals example  are also synthetic. 
            \amits{another point to demonstrate here: when the confound effect is zero, causal effect is identified and our method should show perfect results. }
        \end{enumerate}
        

        \item MNIST34: (Vision dataset) Mouli's paper used this dataset to verify their method. We will use this method for head-to-head comparison with our method:
        \begin{enumerate}
            \item causal topic: color and digit. Final label Y was created using XOR of both the label
            \item spurious topic: rotation (0 or 90), correlated with label
            \item the counterfactuals are also synthetically generated. 
        \end{enumerate}

        \item CivilComments: (NLP dataset) 
        \begin{enumerate}
            \item The main task is to detect toxicity in the sentence
            \item Have three different datasets with different attributes labeled: Gender, Race, and Religion.
            \item Counterfactuals are generated using a manual bag of word removal from sentences. (Not a natural sentence after generating counterfactuals). \abhinav{is the reason for the bad TE estimate due to this?} \amits{is it fast to replace them with gpt-3.5/4 CFs and rerun your method?}
        \end{enumerate}

        \item AAE: (NLP dataset)
        \begin{enumerate}
            \item The main task is to predict the sentiment of the sentence.
            \item The correlated attribute is the race of the person (African-American or Non-Hispanic White)
            \item Counterfactuals are generated using GPT3 (more natural counterfactual).
        \end{enumerate}
        
        
    \end{enumerate}

    \item Baseline:
    \begin{enumerate}
        \item Mouli's Asymmetry Learning Paper \cite{mouli2022asymmetry}: 
        \begin{enumerate}
            \item They used a score based on the predictive accuracy of the invariant model to find the causal vs non-causal topics.
            \item OOD Definition: In their case there the distribution shift is not because of spurious correlation e.g. permutation, rotation, etc. So they automatically find invariance wrt to these transformations.  So, we have shown that when there is a spurious correlation the score they have defined will not work. Also, we need not do causal discovery if our goal is only to find the causal vs spurious attribute. \amits{did not understand this paragraph.}
            \item Dataset to compare: SyntheticNLP, MNIST34, and (possibly) CivilComments \abhinav{TODO: run our setup on MNIST34 and CivilComments on Mouli's method}. 
            \item TODO:
            \begin{enumerate}
                \item Show that their method cannot handle spurious correlation theoretically.
                \item We need to regularize both the causal and spurious topics for a fair comparison. 
            \end{enumerate}
            \amits{what other baselines? we need to finalize the results soon to avoid any surprises.}
        \end{enumerate}
          
    \end{enumerate}

    \item Theoretical Evidence of Robustness to the noise of our method:
    \begin{enumerate}
        \item For one form of regularization: reducing the norm of weights inversely proportional to the treatment effect, theoretical analysis shows that as long as the ranking of treatment effect is correct we we learn a classifier better than ERM. 
        \item TODOs: 
        \begin{enumerate}
            \item Connect the theoretical regularization to the empirical regularization or at least one metric in the result (could use pdelta for that)
            \item Desired solution being global optimum for the multi-feature setting.
        \end{enumerate}
        \item Limitations:
        \begin{enumerate}
            \item Current analysis is for linear models, Later could extend this for general models using kernels, and then infinite-width kernels have a connection with general neural networks. 
        \end{enumerate}
    \end{enumerate}

    \item Empirical Evidence of our Regularization Strategy:
    \begin{enumerate}
        \item Identifying causal vs spurious attributes (Stage 1):
        \begin{enumerate}
            \item  Two estimators:
            \begin{enumerate}
                \item Direct Effect: Simple E(Y|X,T=1) - E(Y|X,T=0). This is expected to be learned by ERM in stage 2 also. So, we should be better or at least equal that this (we will show that even with equal on adding regularization the overall model performs better -- reason unknown, some form of self-regularization or connection from theory on robustness to noise). 
    
                \item RiezNet Estimator: Have two versions: DE (with regularized latent space) and DR (doubly robust estimate). DR is not working correctly across datasets, but DE is better on 2 datasets (SyntheticNLP and AAE) and equivalent on CivilComments. But CivilComment has more resilience to noise so even with incorrect estimates we see a gain in stage 2. 
            \end{enumerate}
            \amits{lets come up with better names to differentiate from ERM. You can call ERM just ERM. Then we can have Reisz(Direct) and Reisz(DR).}
        \end{enumerate}
    
    
        \item Regularizing the models (Stage 2):
        \begin{enumerate}
            \item Our method is able to give gains in OOD even at high correlation but with minor (but expected) drops in the INDO accuracy. \abhinav{need to think of one single metric. GroupDRO paper takes avg accuracy across groups.}\amits{Here's an idea for a single metric. lets create an wt avg accuracy = acc-indistr + $\lambda$ acc-outofdistr. Then compute the lambda range under which our method is better. ERM should be better for zero lambda, groupDRO should be better for $\lambda=1$, but hopefully we can show we cover a wide range in the middle}
            
            \item We see empirical evidence of the resilience to noise in the estimated treatment effect across datasets. Sensitivity is large in AAE but small in other datasets.
            
        \end{enumerate}
    \end{enumerate}
    

\end{enumerate}

==> sections/proof_linear_old.tex <==
\section{Sufficient Condition on Causal Effect Estimation for Learning Robust Model}

\abhinav{TODO: Define the notations formally}

\begin{assumption}[Disentangled latent space]
\label{assm:disentagled_latent}
The latent representation $\bm{z}$ is disentangled and is of form $[\bm{z}_{ca,1},\ldots,\bm{z}_{ca,C},\bm{z}_{sp,1},\ldots,\bm{z}_{sp,S}]$, where  $\{\bm{z}_{ca,k}\in \mathbb{R}^{d_{k}}\}_{k=1}^{C}$ are the features that causally effects the main task label $y$ \abhinav{define this like last time} and $\{\bm{z}_{sp,j}\in \mathbb{R}^{d_{j}}\}_{j=1}^{S}$ are the features spuriously correlated with the main-task label $y$.
Here $d_{k}$ and $d_{j}$ are the dimensions of $\bm{z}_{ca,k}$ and $\bm{z}_{sp,j}$ respectively.  
\end{assumption}


\begin{definition}[Causal Effect Regularization]
\label{def:cereg}
Let $\hat{TE}_{ca,k}$ and $\hat{TE}_{sp,j}$ be the estimated treatment-effect \abhinav{cite} of causal and spuriously correlated feature $\bm{z}_{ca,k}$ and $\bm{z}_{sp,j}$ respectively. Let $h: \bm{z} \rightarrow \bm{y}$ be a linear classifier s.t. $h(\bm{z}) = \sum_{k=1}^{C} \bm{w}_{ca,k} \cdot \bm{z}_{ca,k} + \sum_{j=1}^{S} \bm{w}_{sp,j} \cdot \bm{z}_{sp,j}$. Then we define our causal effect regularization loss as:
\begin{equation*}
    \mathcal{L}_{CEReg}\big{(}h(\bm{z})\big{)} = \mathcal{L}_{mm}\big{(}h(\bm{z})\big{)} + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}_{sp,j}}_{p} \Bigg{\}}
\end{equation*}
where $\mathcal{L}_{mm}$ is the max-margin objective \abhinav{cite}, $R\geq0$ is the regularization strength hyperparameter, $\lambda_{c,k}\propto (\hat{TE}_{ca,k})^{-1}$ and $\lambda_{sp,j} \propto (\hat{TE}_{sp,j})^{-1}$ are the regularization strength for the causal and spurious features $\bm{z}_{ca,k}$ and $\bm{z}_{sp,j}$. Here $\norm{\bm{w}}_{p}$ is the $L_{p}$ norm of the vector $\bm{w}$.
\end{definition}

\begin{remark}
For binary classification task the treatment effect $\hat{TE}_{(\cdot),i}\in[0,1]$ \abhinav{could be negative too if negative correlation. say wlog or that we can always rescale}. Hence, unless otherwise specified, we will use a natural choice to define regularization strength as $\lambda_{(\cdot),i} \coloneqq 1-\hat{TE}_{(\cdot),i}$. \abhinav{state the expected value of lambdas for causal and spurious}
\end{remark}


\begin{theorem}[Sufficient Condition]
\label{theorem:lambda_sufficient}
Let the latent space be frozen and disentangled such that $\bm{z}=[\bm{z}_{ca,1},\ldots,\bm{z}_{ca,C},\bm{z}_{sp,1},\ldots,\bm{z}_{sp,S}]$ (\refassm{assm:disentagled_latent}). Let the classifier trained using max-margin objective be of the form $h^{mm}(\bm{z}) = \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}_{ca,k} + \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}_{sp,j}$ where $\forall k\in[C],\> \bm{w}_{ca,k}^{mm}\neq\bm{0}$ and $\forall j\in[S],\> \bm{w}_{sp,j}^{mm}\neq\bm{0}$ without loss of generality. Let the desired/causal classifier be of form $h^{des}(\bm{z})=\sum_{k=1}^{C} \bm{w}^{des}_{ca,k}\cdot \bm{z}_{ca,k}$ trained using max-margin objective and only uses the causal features $\{\bm{z}_{ca,k}\}_{k=1}^{C}$ for its prediction. Let the norm of the parameters of both the classifier be set to 1 i.e $\sum_{k=1}^{C}\norm{\bm{w}^{mm}_{ca,k}}^{2}_{p=2}+\sum_{j=1}^{S}\norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2} = \sum_{k=1}^{C}\norm{\bm{w}^{des}_{ca,k}}^{2}_{p=2} = 1$.
% Also, let $h^{reg}(\bm{z})=\sum_{k=1}^{C} \bm{w}^{reg}_{ca,k} \cdot \bm{z}_{ca,k} + \sum_{j=1}^{S} \bm{w}^{reg}_{sp,j} \cdot \bm{z}_{sp,j}$ be the classifier trained using our causal effect regularization objective (\refdef{def:cereg}). 
Then if there exists atleast one regularization coefficient of spuriously correlated feature that is not completely incorrect i.e $\exists j\in[S]\> s.t.\> \lambda_{sp,j}\neq0$ and these regularization coefficients are related s.t. $mean_{(k\in[C],j\in[S],\lambda_{sp,j}\neq0)}\big{\{}(\frac{\lambda_{ca,k}}{\lambda_{sp,j}})\cdot \eta_{k,j} \big{\}} < \frac{S^{'}}{C} \cdot \eta$ where $S^{'}=|\{\lambda_{sp,j}: \lambda_{sp,j}\neq0, j\in[S]\}|$, $\eta_{k,j}=\frac{\norm{\bm{w}^{mm}_{ca,k}}_{p}}{\norm{\bm{w}^{mm}_{sp,j}}_{p}}$ and $\eta = \frac{\sum_{k=1}^{C}\norm{\bm{w}^{mm}_{ca,k}}_{p=2}^{2}}{\sum_{j=1}^{S}\norm{\bm{w}^{mm}_{sp,j}}_{p=2}^{2}}$, then for some $\alpha>1$ and $\beta = \sqrt{1+\eta -\eta \alpha^{2}}$, there exist a classifier $h^{\alpha}(\bm{z})=\alpha \big{\{} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}_{ca,k}\big{\}} + \beta \big{\{} \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}_{sp,j} \big{\}}$ s.t

\begin{enumerate}
    \item Assuming existence of unique $h^{des}(\bm{z})$ and $h^{mm}(\bm{z})$,  we have $\hat{\bm{w}}^{des}_{ca,k} = \hat{\bm{w}}^{mm}_{ca,k}$ for all $k\in[C]$, thus $h^{\alpha}(\bm{z})$ is "closer" (\abhinav{make it precise}) to the desired classifier than $h^{mm}(\bm{z})$.
    
    \item  $\beta \cdot \big{(}\sum_{j=1}^{S} \norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2} \big{)} <  \sum_{j=1}^{S}\norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2}$. Thus the classifier $h^{\alpha}(\bm{z})$ relies less on the spurious features than $h^{mm}(\bm{z})$.

    \item $\mathcal{L}_{CEReg}(h^{\alpha}\big{(}\bm{z})\big{)}< \mathcal{L}_{CEReg}\big{(}h^{mm}(\bm{z})\big{)}$. Thus, our causal effect regularization objective (\refdef{def:cereg}) will choose the $h^{\alpha}(\bm{z})$ classifier over the max-margin classifier $h^{mm}(\bm{z})$.

    
\end{enumerate}

\end{theorem}

\begin{remark}
The result of \reftheorem{theorem:lambda_sufficient} holds under a more intuitive but stricter constraint on the regularization coefficient $\lambda$ which states that 
\begin{equation*}
    \lambda_{sp,j} > \Big{(}\frac{S^{'}}{C}\Big{)} \Big{(}\frac{\eta_{k,j}}{\eta}\Big{)} \lambda_{ca,k} \quad\quad\quad \forall k\in[C]\quad \&\quad j\in[S] \abhinav{correct the j index}.
\end{equation*}
\abhinav{define in notation [S] = \{1,...,S\}}. The above constraint states that the regularization strength of the spurious feature should be more than that of the causal feature. Since the regularization strength is inversely proportional to the treatment effect (\refdef{def:cereg}), it states that the treatment effect of the causal feature should be more than that of the spurious feature up to a constant factor. 
\end{remark}





\begin{proof}





\textbf{Proof of Part 1:}
For ease of exposition, we will rewrite the classifiers in equivalent but compact notation. Let the desired classifier (trained using max-margin objective)  $h^{des}(\bm{z})=\sum_{k=1}^{C}\bm{w}^{des}_{ca,k}\cdot \bm{z}_{ca,k}$  be equivalently written in the form $h^{des}(\bm{z}) = \bm{w}^{des}_{ca}\cdot \bm{z}_{ca}$ where $\bm{w}^{des}_{ca} = [\bm{w}^{des}_{ca,1},\ldots,\bm{w}^{des}_{ca,C}]$ and $\bm{z}_{ca} = [\bm{z}_{ca,1},\ldots,\bm{z}_{ca,C}]$. Similarly, let the classifier be trained using the max-margin objective (which uses both causal and spuriously correlated features) $h^{mm}(\bm{z})=\sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}_{ca,k} + \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}_{sp,j}$ be equivalently written as $h^{mm}(\bm{z})= \bm{w}^{mm}_{ca} \cdot \bm{z}_{ca} + \bm{w}^{mm}_{sp} \cdot \bm{z}_{sp}$ where $\bm{w}^{mm}_{ca} = [\bm{w}^{mm}_{ca,1},\ldots,\bm{w}^{mm}_{ca,C}]$, $\bm{z}_{ca} = [\bm{z}_{ca,1},\ldots,\bm{z}_{ca,C}]$, $\bm{w}^{mm}_{sp} = [\bm{w}^{mm}_{sp,1},\ldots,\bm{w}^{mm}_{sp,C}]$ and $\bm{z}_{sp} = [\bm{z}_{sp,1},\ldots,\bm{z}_{sp,C}]$. 

The margin of a classifier $h(\bm{z})$ is given by $\mathcal{M}(h(\bm{z})) = min_{i}\big{\{} \frac{y^{i}h(\bm{z^{i}})}{\norm{h(\bm{z})}} \big{\}}$ where $\bm{z}^{i}$ is the latent representation of $i^{th}$ input datapoint with label $y^{i}$ and $\norm{h(\bm{z})}$ is the norm of the weight vector of the classifier $h(\bm{z})$ (\abhinav{cite preliminary section}). The max-margin objective then maximizes the margin of the given classifier i.e $max_{h(\bm{z})} \mathcal{M}(h(\bm{z}))$ (\abhinav{cite preliminary section}). Since the norm of both $h^{des}(\bm{z})$ and $h^{mm}(\bm{z})$ is $1$, the max-margin objective becomes $max_{h(\bm{z})} min_{i}\big{\{} y^{i}h(\bm{z^{i}}) \big{\}}$.



Now, let $\bm{z}^{des*}$ be the margin point of the desired classifier $h^{des}(\bm{z})$ s.t.:
\begin{equation}
    \begin{aligned}
        \mathcal{M}(h^{des}(\bm{z})) = m(h^{des}(\bm{z}^{des*})) &= y^{des*} \cdot h^{des}(\bm{z}^{des*}) = \underbrace{y^{des*} \cdot \Big{\{} \bm{w}^{des}_{ca}\cdot \bm{z}^{des*}_{ca} \Big{\}}}_{\mathcal{M}^{des}_{ca}}
    \end{aligned}
\end{equation}
Similarly, let $\bm{z}^{mm*}$ be the margin point of the classifier trained using the max-margin objective $h^{mm}(\bm{z})$ s.t.:
\begin{equation}
    \begin{aligned}
        \mathcal{M}(h^{mm}(\bm{z})) = m(h^{mm}(\bm{z}^{mm*})) &= y^{mm*} \cdot h^{mm}(\bm{z}^{mm*})\\
        &=\underbrace{  y^{mm*} \cdot \Big{\{} \bm{w}^{mm}_{ca}\cdot \bm{z}^{mm*}_{ca} \Big{\}}}_{\mathcal{M}^{mm}_{ca}} +  y^{mm*} \cdot \Big{\{}  \bm{w}^{mm}_{sp} \cdot \bm{z}^{mm*}_{sp} \Big{\}}\\
    \end{aligned}
\end{equation}
We will use proof by contradiction to show that $\bm{w}_{ca}^{mm}=\bm{w}_{ca}^{des}$. 

\textbf{Contradiction Assumption}: Let's assume that $\bm{w}_{ca}^{mm}\neq\bm{w}_{ca}^{des}$. From the statement of the first part of this theorem, there is a unique $h^{des}(\bm{z})$ and $h^{mm}(\bm{z})$. Given $\bm{w}_{ca}^{mm}\neq\bm{w}_{ca}^{des}$, we cannot have $\mathcal{M}_{ca}^{des}=\mathcal{M}_{ca}^{mm}$, otherwise we will have multiple solution for $h^{des}(\bm{z})$ where both $\bm{w}^{des}_{ca}$ and $\bm{w}^{mm}_{ca}$ gives same max-margin objective.
Now we have the following two cases based on the value of $\mathcal{M}^{des}_{ca}$ and $\mathcal{M}^{mm}_{ca}$.

\textbf{Case 1} ($\mathcal{M}^{des}_{ca}$ > $\mathcal{M}^{mm}_{ca}$): 
Since $\bm{z}^{des*}$ is the margin point of $h^{des}(\bm{z})$, we have:
\begin{equation}
    \begin{aligned}
        y^{des*}\cdot \Big{\{} \bm{w}^{des}_{ca}\cdot \bm{z}^{des*}_{ca} \Big{\}} &< y^{t}\cdot \Big{\{} \bm{w}^{des}_{ca}\cdot \bm{z}^{t}_{ca} \Big{\}}  \quad \forall \bm{z}^{t}\neq \bm{z}^{des*} \\
    \end{aligned}
\end{equation}
Next, since  $\mathcal{M}^{des}_{ca}$ > $\mathcal{M}^{mm}_{ca}$, using above equation we have:
\begin{equation}
\label{eq:part1_case1_mm_des_ineq}
    \begin{aligned}
         y^{mm*} \cdot \Big{\{} \bm{w}^{mm}_{ca}\cdot \bm{z}^{mm*}_{ca} \Big{\}} &< y^{t}\cdot \Big{\{} \bm{w}^{des}_{ca}\cdot \bm{z}^{t}_{ca} \Big{\}}  \quad \forall \bm{z}^{t} \\
    \end{aligned}
\end{equation}
Also, since $\bm{z}^{mm*}$ is the margin point of $h^{mm}(\bm{z})$, $\forall \bm{z}^{t}\neq \bm{z}^{mm*}$ we have:
\begin{equation}
\label{eq:part1_case1_mm_point_ineq}
    y^{mm*} \cdot \Big{\{} \bm{w}^{mm}_{ca}\cdot \bm{z}^{mm*}_{ca} \Big{\}} +  y^{mm*} \cdot \Big{\{}  \bm{w}^{mm}_{sp} \cdot \bm{z}^{mm*}_{sp} \Big{\}} < y^{t} \cdot \Big{\{} \bm{w}^{mm}_{ca}\cdot \bm{z}^{t}_{ca} \Big{\}} +  y^{t} \cdot \Big{\{}  \bm{w}^{mm}_{sp} \cdot \bm{z}^{t}_{sp} \Big{\}} \\
\end{equation}
Using \refeqn{eq:part1_case1_mm_des_ineq} and \refeqn{eq:part1_case1_mm_point_ineq}, $\forall \bm{z}^{t}\neq \bm{z}^{mm*}$ we have:
\begin{equation}
    \begin{aligned}
        y^{mm*} \cdot \Big{\{} \bm{w}^{mm}_{ca}\cdot \bm{z}^{mm*}_{ca} \Big{\}} +  y^{mm*} \cdot \Big{\{}  \bm{w}^{mm}_{sp} \cdot \bm{z}^{mm*}_{sp} \Big{\}}
    \end{aligned}
\end{equation}



\textbf{Case 2} ($\mathcal{M}^{des}_{ca}$ < $\mathcal{M}^{mm}_{ca}$): 










\textbf{Proof of Part 2:}
The norm of the spurious component of the classifier $h^{\alpha}(\bm{z})$ is equal to $\beta \cdot \big{(}\sum_{j=1}^{S} \norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2}\big{)}$ and the norm of the spurious component of the classifier $h^{mm}(\bm{z})$ is equal to $\sum_{j=1}^{S}\norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2}$. Next, we have 
\begin{equation}
    \beta = \sqrt{1+\eta -\eta \alpha^{2}} = \sqrt{1+\eta (1-\alpha^{2})} <1
\end{equation}
since $\eta>0$ 
\abhinav{Can $\eta$ be equal to zero? This will happen when the causal feature is not used at all. No not possible from the first statement of this theorem. Then $\eta =0$ and $\beta=1$!!}   and $\alpha>1$ (from the statement of \reftheorem{theorem:lambda_sufficient}). Thus $\beta \cdot \big{(}\sum_{j=1}^{S} \norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2} \big{)} <  \sum_{j=1}^{S}\norm{ \bm{w}^{mm}_{sp,j}}_{p=2}^{2}$ completing the first part of the proof. 










\textbf{Proof of Part 3:}
We will show that there always exists a regularization strength $R\geq0$ s.t. $\mathcal{L}_{CEReg}(h^{\alpha}\big{(}\bm{z})\big{)}< \mathcal{L}_{CEReg}\big{(}h^{mm}(\bm{z})\big{)}$ given $mean_{(k,j)}\big{\{}(\frac{\lambda_{ca,k}}{\lambda_{sp,j}})\cdot \eta_{k,j} \big{\}} < \frac{S^{'}}{C} \cdot \eta$ (from the main statement of \reftheorem{theorem:lambda_sufficient}). To have $\mathcal{L}_{CEReg}(h^{\alpha}\big{(}\bm{z})\big{)}< \mathcal{L}_{CEReg}\big{(}h^{mm}(\bm{z})\big{)}$ we need to select the regularization strength $R\geq0$ s.t:
\begin{equation}
\label{eq:claim2_loss_compare}
\begin{aligned}
    \mathcal{L}_{mm}\big{(}h^{\alpha}(\bm{z})\big{)} + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \alpha \norm{\bm{w}^{mm}_{ca,k}}_{p} &+ \sum_{j=1}^{S} \lambda_{sp,j} \beta  \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}} < \\
    &\mathcal{L}_{mm}\big{(}h^{mm}(\bm{z})\big{)} + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}}
\end{aligned}
\end{equation}
The max-margin objective given is given by (\abhinav{cite/add preliminary section}) $\mathcal{L}_{mm}\big{(}h(\bm{z})\big{)} = (-1)\cdot \min_{i} \big{\{}\frac{y^{i}h(\bm{z}^{i})}{\norm{h(\bm{z})}}\big{\}}$ where $\bm{z}^{i}$ is the latent representation of $i^{th}$ input datapoint with label $y^{i}$ and $\norm{h(\bm{z})}$ is the norm of the weight vector of the classifier $h(\bm{z})$. The norm of classifier $h^{mm}(\bm{z})$ is $1$ (from the statement of this \reftheorem{theorem:lambda_sufficient}) and the norm of the classifier $h^{\alpha}(\bm{z})$ is:
\begin{equation}
\begin{aligned}
        \norm{h^{\alpha}(\bm{z})} &= \alpha^{2} \sum_{k=1}^{C}  \norm{\bm{w}^{mm}_{ca,k}}^{2}_{p=2} + \beta^{2}  \sum_{j=1}^{S}  \norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2}\\
        &= \alpha^{2} \sum_{k=1}^{C}  \norm{\bm{w}^{mm}_{ca,k}}^{2}_{p=2} + (1+\eta-\eta \alpha^{2}) \sum_{j=1}^{S}  \norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2}\\
        &= \alpha^{2} \sum_{k=1}^{C}  \norm{\bm{w}^{mm}_{ca,k}}^{2}_{p=2} + (1 - \alpha^{2}) \frac{\sum_{k=1}^{C}\norm{\bm{w}^{mm}_{ca,k}}_{p=2}^{2}}{\cancel{\sum_{j=1}^{S}\norm{\bm{w}^{mm}_{sp,j}}_{p=2}^{2}}} \Bigg{\{}\cancel{\sum_{j=1}^{S}  \norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2}}\Bigg{\}} + \sum_{j=1}^{S}  \norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2}  \\
        &= \sum_{k=1}^{C}  \norm{\bm{w}^{mm}_{ca,k}}^{2}_{p=2} + \sum_{j=1}^{S}  \norm{\bm{w}^{mm}_{sp,j}}^{2}_{p=2} = 1 \\
\end{aligned}
\end{equation} 
Substituting the max-margin loss for both the classifier in \refeqn{eq:claim2_loss_compare} we get:
\begin{equation}
\label{eq:claim2_mm_subs}
\begin{aligned}
    (-1) \cdot min_{i}\Big{\{} y^{i} h^{\alpha}(\bm{z}^{i}) \Big{\}} + R \cdot \Bigg{\{} \sum_{k=1}^{C} & \lambda_{ca,k} \alpha \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \beta  \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}} < \\
    & (-1) \cdot min_{j}\Big{\{} y^{j} h^{mm}(\bm{z}^{j}) \Big{\}} + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}}
\end{aligned}
\end{equation}
Next, we will show that there always exists an $R\geq 0$ for a stronger inequality, when satisfied, also implies that the above \refeqn{eq:claim2_mm_subs} is also satisfied. Let $\bm{z}^{t}$ be the latent representation of the $t^{th}$ datapoint such that $t=argmin_{i}\Big{\{} y^{i} h^{\alpha}(\bm{z}^{i}) \Big{\}}$, then we will show that there always exists $R\geq 0$ the following inequality is satisfied given $mean_{(k,j)}\big{\{}(\frac{\lambda_{ca,k}}{\lambda_{sp,j}})\cdot \eta_{k,j} \big{\}} < \frac{S^{'}}{C} \cdot \eta$:
\begin{equation}
\label{eq:claim2_same_datapoint_inequality}
\begin{aligned}
    -y^{t} h^{\alpha}(\bm{z}^{t}) + R \cdot \Bigg{\{} \sum_{k=1}^{C} & \lambda_{ca,k} \alpha \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \beta  \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}} < \\
    &  -y^{t} h^{mm}(\bm{z}^{t}) + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}}
\end{aligned}
\end{equation}
Since $(-1)\cdot min_{j}\Big{\{} y^{j} h^{mm}(\bm{z}^{j}) \Big{\}} \geq - y^{k} h^{\alpha}(\bm{z}^{t}) $ (\abhinav{verify this again}), the values of $R$ that will satisfy \refeqn{eq:claim2_same_datapoint_inequality} will also satisfy \refeqn{eq:claim2_mm_subs}. Next, substituting $h^{\alpha}(\bm{z}^{t})$ and $h^{mm}(\bm{z}^{t})$ in \refeqn{eq:claim2_same_datapoint_inequality} we get:
\begin{equation}
\begin{aligned}
    -y^{t} & \Bigg{\{} \alpha \big{\{} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k}\big{\}} + \beta \big{\{} \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} \big{\}} \Bigg{\}}  + R \cdot \Bigg{\{} \sum_{k=1}^{C}  \lambda_{ca,k} \alpha \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \beta  \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}} < \\
    &  -y^{t}  \Bigg{\{}  \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k} +  \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} \Bigg{\}} + R \cdot \Bigg{\{} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p} + \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} \Bigg{\}}
\end{aligned}
\end{equation}
\abhinav{add more steps}
since $\alpha>1$ and $0\leq\beta<1$ (\abhinav{cite from claim 2.}), rearranging we get:
\begin{equation}
\label{eq:claim2_final_r_inequality}
    \begin{aligned}
        \implies &(\alpha-1) \Bigg{\{} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k} - R \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}  \Bigg{\}} > (1-\beta) \Bigg{\{}  \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} - R \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p}  \Bigg{\}}\\
        \implies & \frac{(\alpha-1)}{(1-\beta)}  \Bigg{\{} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k} - R \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}  \Bigg{\}} >  \Bigg{\{}  \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} - R \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p}  \Bigg{\}}\\
        \implies & R \cdot \Bigg{\{} \underbrace{ \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} -  \frac{(\alpha-1)}{(1-\beta)} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}}_{\text{LHS-term 1}}   \Bigg{\}} > \Bigg{\{} \underbrace{\sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} -  \frac{(\alpha-1)}{(1-\beta)} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k}}_{\text{RHS-term 2}} \Bigg{\}}\\
    \end{aligned}
\end{equation}
If the LHS-term 1 in the above equation is greater than $0$, then we can always select a regularization strength $R>0$ s.t. the above inequality is always satisfied, whenever
\begin{equation}
\label{eq:claim2_r_condition}
    R > \frac{\Bigg{\{} \sum_{j=1}^{S} \bm{w}^{mm}_{sp,j} \cdot \bm{z}^{t}_{sp,j} -  \frac{(\alpha-1)}{(1-\beta)} \sum_{k=1}^{C} \bm{w}^{mm}_{ca,k} \cdot \bm{z}^{t}_{ca,k} \Bigg{\}}}{\Bigg{\{}  \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} -   \frac{(\alpha-1)}{(1-\beta)} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}   \Bigg{\}}}
\end{equation}
Next we will show that given $mean_{(k,j)}\big{\{}(\frac{\lambda_{ca,k}}{\lambda_{sp,j}})\cdot \eta_{k,j} \big{\}} < \frac{S^{'}}{C} \cdot \eta$, the term 1 in \refeqn{eq:claim2_final_r_inequality} is always greater than 0. For term 1 to be greater than 0 we need: 
\begin{equation}
\begin{aligned}
    \sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p} &>  \frac{(\alpha-1)}{(1-\beta)} \sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}\\
    % \sum_{j=1}^{S} \frac{\lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p}}{\sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}} &> \frac{(\alpha-1)}{(1-\beta)} 
\end{aligned}
\end{equation}
Next, we have the following two cases for possible value $\lambda_{ca,k}$ can take:

\textbf{Case 1} $\big{(}\lambda_{ca,k}=0,\> \forall k\in[C]\big{)}$: 
For this case the above equation is trivially satisfied i.e $\sum_{j=1}^{S} \lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p}>0$ since $\norm{\bm{w}_{sp,j}^{mm}}_{p}\neq0$ and $\exists j\in[S] \> s.t. \> \lambda_{sp,j}\neq 0 $ (from the statement of this \reftheorem{theorem:lambda_sufficient}). 

\textbf{Case 2} $\big{(}\exists k\in[C], \> s.t.\> \lambda_{ca,k}\neq0\big{)}$: Since $\norm{\bm{w}_{ca,k}^{mm}}_{p}>0$ for all $k\in[C]$ (from the statement of this theorem), we have $\sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}>0$.  Recalling from the main statement of this theorem, $S^{'}=|\{\lambda_{sp,j} | \lambda_{sp,j}\neq0, j\in[S]\}|$ be the number of spuriously correlated feature's regularization coefficient that is non-zero, then again rearranging we get:
\begin{equation}
\begin{aligned}
    \sum_{j=1}^{S} \frac{\lambda_{sp,j} \norm{\bm{w}^{mm}_{sp,j}}_{p}}{\sum_{k=1}^{C} \lambda_{ca,k} \norm{\bm{w}^{mm}_{ca,k}}_{p}} &> \frac{(\alpha-1)}{(1-\beta)} \\
    \sum_{j=1,\lambda_{sp,j}\neq0}^{S} \frac{1}{\sum_{k=1}^{C}\big{(}\frac{\lambda_{ca,k}}{\lambda_{sp,j}}\big{)} \big{(}\frac{\norm{\bm{w}_{ca,k}^{mm}}_{p}}{\norm{\bm{w}_{sp,j}^{mm}}_{p}}\big{)}} &>\frac{(\alpha-1)}{(1-\beta)}\\
    \frac{1}{\sum_{j=1,\lambda_{sp,j}\neq0}^{S} \Bigg{\{} \underbrace{\frac{1}{\sum_{k=1}^{C}\big{(}\frac{\lambda_{ca,k}}{\lambda_{sp,j}}\big{)} \big{(}\frac{\norm{\bm{w}_{ca,k}^{mm}}_{p}}{\norm{\bm{w}_{sp,j}^{mm}}_{p}}\big{)}}}_{\text{LHS-term 3}} \Bigg{\}}} \cdot S^{'} &< \frac{(1-\beta)}{(\alpha-1)} \cdot S^{'}
\end{aligned}
\end{equation}
The above equation is the harmonic mean of the LHS-term 3 and LHS-term 3 is $\geq0$ for all values of $j$. We know that the harmonic mean is always less than equal to the arithmetic mean for a set of positive numbers (\abhinav{cite}).  Thus the above inequality is satisfied if:
\begin{equation}
\label{eq:claim2_lambda_alpha_ineqality}
\begin{aligned}
    \sum_{j=1,\lambda_{sp,j}\neq0}^{S}\sum_{k=1}^{C} \frac{\big{(}\frac{\lambda_{ca,k}}{\lambda_{sp,j}}\big{)} \big{(}\frac{\norm{\bm{w}_{ca,k}^{mm}}_{p}}{\norm{\bm{w}_{sp,j}^{mm}}_{p}}\big{)}}{S^{'}\cdot C} <  \frac{(1-\beta)}{(\alpha-1)} \cdot \frac{S^{'}}{C}
\end{aligned}
\end{equation}
Next, we will make use of the following lemma to show that the term $\frac{1-\beta}{\alpha-1}>\eta$ where $\eta = \frac{\sum_{k=1}^{C}\norm{\bm{w}^{mm}_{ca,k}}_{p=2}^{2}}{\sum_{j=1}^{S}\norm{\bm{w}^{mm}_{sp,j}}_{p=2}^{2}}$ (define the main statement of this theorem). 
The proof of this lemma can be found after the end of the proof of this theorem. 
\begin{lemma}
\label{lemma:beta_by_alpha_lb}
The function $f(\alpha) = \frac{1-\beta}{\alpha-1}=\frac{\sqrt{1+\eta-\eta\alpha^{2}}}{\alpha-1}$ is a monotonically increasing function for $\alpha>1$ and $f(\alpha) > \eta$ for all $\alpha>1$.
\end{lemma}

From \reflemma{lemma:beta_by_alpha_lb} we have $\frac{1-\beta}{\alpha-1}>\eta$ for $\alpha>1$. Thus the inequality in \ref{eq:claim2_lambda_alpha_ineqality} is satisfied if the regularization strength of features ($\lambda$) satisfies the following condition:
\begin{equation}
\begin{aligned}
    \sum_{j=1,\lambda_{sp,j}\neq0}^{S}\sum_{k=1}^{C} \frac{\big{(}\frac{\lambda_{ca,k}}{\lambda_{sp,j}}\big{)} \big{(}\frac{\norm{\bm{w}_{ca,k}^{mm}}_{p}}{\norm{\bm{w}_{sp,j}^{mm}}_{p}}\big{)}}{S^{'}\cdot C} <  \eta \cdot \frac{S^{'}}{C}\\
    mean_{(j,k,\lambda_{sp,j}\neq0)} \Big{\{} (\frac{\lambda_{ca,k}}{\lambda_{sp,j}})\cdot \eta_{k,j} \big{\}} \Big{\}} < \eta \cdot \frac{S^{'}}{C}\\
\end{aligned}
\end{equation}
where $\eta_{k,j} = \frac{\norm{\bm{w}_{ca,k}^{mm}}_{p}}{\norm{\bm{w}_{sp,j}^{mm}}_{p}}$. Since the above condition on regularization strength of features are satisfied (given in the main statement of this theorem), we have $\mathcal{L}_{CEReg}(h^{\alpha}\big{(}\bm{z})\big{)}< \mathcal{L}_{CEReg}\big{(}h^{mm}(\bm{z})\big{)}$ thus completing the proof.

\end{proof}




\begin{proof}[Proof of \reflemma{lemma:beta_by_alpha_lb}]
Taking the derivative of $f(\alpha)$ we get:
\begin{equation}
\label{eq:df_by_dalpha}
\begin{aligned}
    \frac{d \Big{(}\frac{1-\beta}{\alpha-1} \Big{)}}{d \alpha} &=  \frac{d \Big{(}\frac{1-\sqrt{1+\eta-\eta \alpha^{2}}}{\alpha-1}\Big{)}}{d \alpha}\\
    &=\frac{\frac{(\alpha-1)\eta \alpha}{\sqrt{1+\eta-\eta\alpha^{2}}} - (1-\sqrt{1+\eta -\eta\alpha^{2}}) }{(\alpha-1)^{2}}\\
    &=\frac{\frac{(\alpha-1)\eta\alpha}{\beta}-(1-\beta)}{(\alpha-1)^{2}}
\end{aligned}
\end{equation}
We have $\beta=\sqrt{1+\eta - \eta \alpha^{2}} = \sqrt{1+\eta(1-\alpha^{2})}<1$ since $\eta>0$ (\abhinav{cite from the first claim}) and $\alpha>1$ (from the main statement of \reftheorem{theorem:lambda_sufficient}). Also as $\alpha$ increases $\beta$ decreases, and since $\beta\geq 0$ we have an upper limit on the value of $\alpha$. Thus $\alpha\in(1,\alpha_{max}]$ where $\alpha_{max}$ is given by:
\begin{equation}
\begin{aligned}
    \beta = & \sqrt{1+\eta-\eta\alpha_{max}^{2})} = 0\\ 
    \implies & 1+\eta-\eta\alpha_{max}^{2} = 0\\
    \implies & \alpha_{max} = \sqrt{\frac{1+\eta}{\eta}}
\end{aligned} 
\end{equation}

\textbf{Case 1} ($\beta=0$):
We have $\alpha = \alpha_{max}>1$ and when $\beta=0$, $\frac{df(\alpha)}{d\alpha} = \infty > 0$ (from \refeqn{eq:df_by_dalpha}).

\textbf{Case 2} ($\beta\in(0,1)$): The denominator is greater than 0 since $\alpha\in(1,\alpha_{max})$. Next, we will show that the numerator is also greater than  zero for all $\alpha\in(1,\alpha_{max})$ which will imply that the $\frac{d f(\alpha)}{d\alpha}>0$. Thus $f(\alpha)$ is a monotonically increasing function for $\alpha\in(1,\alpha_{max})$. For the numerator of the above equation to be positive we need:
\begin{equation}
\label{eq:claim2_numerator_positive_inequality}
\begin{aligned}
    &\implies \frac{(\alpha-1)\eta \alpha}{\beta} - (1-\beta) > 0 \\
    &\implies \frac{(\alpha-1)\eta\alpha - \beta + \beta^{2}}{\beta} >0\\
    &\implies \cancel{\eta \alpha^{2}} -\eta\alpha + 1 + \eta -\cancel{\eta\alpha^{2}} - \beta >0\\
    &\implies 1+ \eta -\eta \alpha  > \beta \\
\end{aligned}
\end{equation}
% Since $\eta >0$ (\abhinav{cite from the first claim}), the above inequality is always true for all values of $\alpha>1$ since:
% \begin{equation}
%     \begin{aligned}
%         1+\eta-\eta\alpha > 1+\eta -\eta \alpha^{2}\\
%         \implies 1+\eta -\eta\alpha > \sqrt{}
%     \end{aligned}
% \end{equation}
The LHS of the above equation is always positive since:
\begin{equation}
    \begin{aligned}
        \alpha &< \alpha_{max} = \sqrt{\frac{1+\eta}{\eta}} \\ 
        \implies\alpha &< \frac{1+\eta}{\eta}\\
        \implies \eta\alpha &< 1+\eta\\
        \implies 0 &< 1+\eta -\eta\alpha
    \end{aligned}
\end{equation}
Thus squaring both side in \refeqn{eq:claim2_numerator_positive_inequality} we get:
\begin{equation}
    \begin{aligned}
        &\implies \cancel{1}+\eta^{{2}}+2{\eta} + \eta^{{2}}\alpha^{2} -2(\eta+1)({\eta}\alpha)> \cancel{1}+{\eta} -1{\eta} \alpha^{2}\\
        &\implies \eta^{\cancel{2}}+2\cancel{\eta} + \eta^{\cancel{2}}\alpha^{2} -2(\eta+1)(\cancel{\eta}\alpha)> 1\cancel{\eta} -\cancel{\eta} \alpha^{2}\\
        &\implies (\eta+1) \alpha^{2} - 2(\eta+1)\alpha + (\eta +1)>0\\
        &\implies (\eta+1) (\alpha^{2}-2\alpha +1) >0\\
        &\implies (\eta+1) (\alpha-1)^{2}>0\\
        &\implies \alpha>1
    \end{aligned}
\end{equation}
Thus from both Case 1 and Case 2, for all values of $\alpha \in (1,\alpha_{max}]$ we have $\frac{d f(\alpha)}{d\alpha}>0 \implies $ $f(\alpha)$ is an increasing function. Next, we will show that $f(\alpha=1) = \eta$, thus $f(\alpha)>\eta$ for all $\alpha>1$ since $f(\alpha)$ is an increasing function thereby completing the proof. We have:
\begin{equation}
    \begin{aligned}
        f(\alpha=1) &= \lim_{\alpha \to 1} \frac{1-\beta}{\alpha-1}\\
        &= \lim_{\alpha \to 1} \frac{\frac{\eta \alpha}{\sqrt{1+\eta-\eta\alpha^{2}}}}{1} = \eta   \quad (\text{L'H}\hat{o}\text{pital rule})\\ 
    \end{aligned}
\end{equation}



 

\end{proof}




==> sections/todo.tex <==
Things commented out. Consider moving to appendix. 

%We assume access to the counterfactual inputs with the desired \prop changed but no access to the corresponding main task label. % for these examples though. 

% We use an average of pretrained GloVe embeddings \cite{pennington2014glove} of words in the sentence as the default encoder for this dataset. 


MNIST The counterfactual examples for a specific \prop (color or rotation) are generated by deterministic transformation of those \props in the image. Unlike \syn dataset, we leave both the causal features in the input but digit \prop is not used in any of our experiments. 

Given a set of \props, Mouli+CAD \cite{mouli2022asymmetry} defines a score (see \refappendix{appendix:math_preliminaries}) to find the subset of \props that do not causally affect the main task label $y_{m}$ and hence  are spurious.

In \synuc dataset at the high predictive correlation ($\kappa>0.7$) even though the causal effect of spurious \prop is not completely correct, \oursshort will not treat it as completely causal whereas \mouli will detect it as causal (see \reffig{fig:mouli_score_syn_mnist_aae} and discussion above). Similarly for \mnist dataset \mouli will incorrectly detect the spurious \prop (rotation) as causal for all $\kappa$ whereas \oursshort will use the causal effect of rotation ($\leq0.31$ for all $\kappa$) which is close to true value $0$.
